Text Compression using Abstract Numeration System on a Regular Language

An abstract numeration system (ANS) is a numeration system that provides a one-to-one correspondence between the natural numbers and a regular language. In this paper, we define an ANS-based compression as an extension of this correspondence. In addition, we show the following results: 1) an average compression ratio is computable from a language, 2) an ANS-based compression runs in sublinear time with respect to the length of the input string, and 3) an ANS-based compression can be extended to block-based compression using a factorial language.

==> macros.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input :}}
\renewcommand{\algorithmicensure}{\textbf{Output :}}

\renewcommand{\algorithmiccomment}[1]{// #1}
\makeatletter
\def\endfor{\end{ALC@for}}
\def\endif{\end{ALC@if}}
\def\endwhile{\end{ALC@while}}
\makeatother

\newcommand{\powerset}{\mathfrak{P}}
\newcommand{\mapping}{\mathfrak{F}}
\newcommand{\so}{.\raisebox{1ex}{.}.}  
\newcommand{\ed}{$\hfill\diamond$}
\newcommand{\ued}{\begin{flushright}\raisebox{5ex}[1ex][0ex]{{\smash
				  \ed}}\end{flushright}\vspace{-5ex}}
\newcommand{\uqed}{\begin{flushright}\raisebox{5ex}[1ex][0ex]{{\smash
				  \qed}}\end{flushright}\vspace{-5ex}}

\makeatletter
\newcommand{\figcaption}[1]{\def\@captype{figure}\caption{#1}}
\newcommand{\tblcaption}[1]{\def\@captype{table}\caption{#1}}
\makeatother

\def\CA{{\cal A}}
\def\CN{{\cal N}}
\def\CD{{\cal D}}
\def\CU{{\cal U}}
\def\CS{{\cal S}}

\newtheorem{fact}{Fact}

\newcommand{\NFA}{\mathop{\mathrm{NFA}}\nolimits}
\newcommand{\DFA}{\mathop{\mathrm{DFA}}\nolimits}
\newcommand{\UFA}{\mathop{\mathrm{UFA}}\nolimits}

\newcommand{\suc}{\mathop{\mathrm{suc}}\nolimits}
\newcommand{\pre}{\mathop{\mathrm{pre}}\nolimits}
\newcommand{\val}{\mathop{\mathrm{val}}\nolimits}
\newcommand{\rep}{\mathop{\mathrm{rep}}\nolimits}

\newcommand{\order}{\mathrm{O}}
\newcommand{\mult}{\mathfrak{M}}
\newcommand{\mmult}{\mathfrak{MM}}
\newcommand{\pd}[1]{{{\mathrm{Pd}}(#1)}}
\newcommand{\ind}{\mathrm{Ind}}
\newcommand{\fac}{\mathop{\mathrm{FACT}}\nolimits}
\newcommand{\bool}{\mathbb{B}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\real}{\mathbb{R^+}}
\newcommand{\conv}[2]{{\cal B}_{#1 \rightarrow #2}}
\newcommand{\Conv}[2]{\mathop{\cal B}\limits_{#1 \rightarrow #2}}
\newcommand{\ratio}{\mathrm{CR}}
